Constrained Synchronization and Subset Synchronization Problems for Weakly Acyclic Automata

We investigate the constrained synchronization problem for weakly acyclic, or partially ordered, input automata. We show that, for input automata of this type, the problem is always in NP. Furthermore, we give a full classification of the realizable complexities for constraint automata with at most two states and over a ternary alphabet. We find that most constrained problems that are PSPACE-complete in general become NP-complete. However, there also exist constrained problems that are PSPACE-complete in the general setting but become polynomial time solvable when considered for weakly acyclic input automata. We also investigate two problems related to subset synchronization, namely if there exists a word mapping all states into a given target subset of states, and if there exists a word mapping one subset into another. Both problems are PSPACE-complete in general, but in our setting the former is polynomial time solvable and the latter is NP-complete.

==> small_pto.tex <==
\section{Monotonic Constraint Automata with Three States and Arbitrary Alphabet}

%
% 2 zustände immer monoton, also noch beliebige zustände.
%
% binäres alphabet immer in np, und nur eine situation wenn in mitte schleife mti NP-c
% annehmen connected, final 3, allgemein partially ordered F maximale
%
% |Sigma_{n,n}| \le 1, da über ternären alphabet sonst P [wenn alle] oder pspace wenn eins nicht
%
% allgemein (a+b)^*uSigma_{3,3} mit allen sigma_{i,i} leer psspace hard mit Cu-Theorem?

\subsection{Totally Ordered}

\begin{proposition}
 If $|\Sigma_{1,1}| \ge 2$, then pspace hard
\end{proposition}
\begin{proof}
 Let $a,b \in \Sigma_{1,1}$ be distinct and $c \in \Sigma_{1,2}$
 and $d \in \Sigma_{2,3}$.
 %If $\{c,d\}\cap \Sigma_{3,3} = \emptyset$,
 Then, note that $c \notin \Sigma_{1,1}$, we have $\Sigma^*acd\Sigma^* \cap L(\mathcal B) = \Sigma_{1,1}^*acd\Sigma_{3,3}^*$.
%  if $c \in \Sigma_{2,2}$
%  or it equals $\Sigma_{1,1}^*cc^*d\Sigma_{3,3}^*$
%  otherwise.
 
 
 
 
\end{proof}


\begin{proposition}
 If $|\Sigma_{2,2}| \ge 2$, then pspace hard
\end{proposition}
\begin{proof}
 %Sigma_{1,1} kleiner 1 annehmen
 %
 % two state und davor Sigma_{1,1}\Sigma_{1,2} kopie davorschalten -> geht allgemein! induktiv ??
 %
 % mit totally ordered geht sowas davor wenn alphabete disunkt
\end{proof}
